What Color Scheme is More Effective in Assisting Readers to Locate Information in a Color-Coded Article?

Color coding, a technique assigning specific colors to cluster information types, has proven advantages in aiding human cognitive activities, especially reading and comprehension. The rise of Large Language Models (LLMs) has streamlined document coding, enabling simple automatic text labeling with various schemes. This has the potential to make color-coding more accessible and benefit more users. However, the impact of color choice on information seeking is understudied. We conducted a user study assessing various color schemes' effectiveness in LLM-coded text documents, standardizing contrast ratios to approximately 5.55:1 across schemes. Participants performed timed information-seeking tasks in color-coded scholarly abstracts. Results showed non-analogous and yellow-inclusive color schemes improved performance, with the latter also being more preferred by participants. These findings can inform better color scheme choices for text annotation. As LLMs advance document coding, we advocate for more research focusing on the "color" aspect of color-coding techniques.

==> Figures/bar-chart-figures.tex <==
\begin{figure*}[t]
    \centering
    
    \begin{subfigure}{0.31\textwidth}
        \centering
    \includegraphics[width=\textwidth]{Figures/bar-chart/bar_chart_Response Rate.png}
    \caption{Response Rate Bar Chart}
    \label{fig:bar_response}
    \end{subfigure}
    \hspace{2mm}
    \begin{subfigure}{0.31\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/bar-chart/bar_chart_ACC.png}
    \caption{ACC Bar Chart}
    \label{fig:bar_acc}
    \end{subfigure}
    \hspace{2mm}
    \begin{subfigure}{0.31\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/bar-chart/bar_chart_Duration.png}
    \caption{Duration Bar Chart}
    \label{fig:bar_duration}
    \end{subfigure}
    \caption{User study results.}
    \label{fig:bar_charts}
    %\kenneth{TODOs: (1) Just white background with NO grid lines, (2) add error bar}\steven{done. error bar is using 95\% confidence interval}
\end{figure*}

==> Figures/demo-figures.tex <==
\begin{figure*}[t]
    \centering
    
    \begin{subfigure}{0.8\textheight}
        \centering
    \includegraphics[width=\textwidth]{Figures/demo_interface/color-palette-demo-1.png}
    \caption{\textbf{Sequential} color scheme used in the study.}
    \label{fig:demo_1}
    \end{subfigure}
    
    \vspace{2mm}
    
    \begin{subfigure}{0.8\textheight}
    \centering
    \includegraphics[width=\textwidth]{Figures/demo_interface/color-palette-demo-2.png}
    \caption{\textbf{Diverging} color scheme used in the study.}
    \label{fig:demo_2}
    \end{subfigure}
    
    \vspace{2mm}
    
    \begin{subfigure}{0.8\textheight}
    \centering
    \includegraphics[width=\textwidth]{Figures/demo_interface/color-palette-demo-3.png}
    \caption{\textbf{Qualitative} color scheme used in the study.}
    \label{fig:demo_3}
    \end{subfigure}
    \vspace{-.5pc}
    \caption{A sample abstract that is color-coded by three color schemes. Along the right side, the labels - Background, Purpose, Method, Finding, and Other - are arranged from top to bottom for each color scheme.}
    \vspace{-1pc}
    \label{fig:demo_articles}
\end{figure*}

%\kenneth{TODO: (1) Mention ``sequential, diverging, qualitative'', (2) Can we be even more specific, e.g., list the code of each color?, (3) Don't need to show the label here maybe}\steven{done}

==> Figures/user-rating.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{Figures/rating-chart/bar_chart_post_survey_type.png}
    \includegraphics[width=0.59\linewidth]{Figures/rating-chart/bar_chart_post_survey_stacked.png}
    \vspace{-.5pc}
    \caption{The user rating towards different color schemes.}
    \vspace{-.5pc}
    \label{fig:user_rating}
\end{figure}

%\kenneth{TODOs: (1) The whole paper's figures should use the same color for Seq/Divergin/Qual bars. (2) The fonts of these figures should be larger. (3) Can you make these charts more flat by reducing the spaces between the bars?}\steven{done}

% \begin{figure*}[t]
%     % \centering
%     \begin{subfigure}{0.40\textwidth}
%     % \centering
%     \includegraphics[height=2cm,keepaspectratio]{Figures/rating-chart/bar_chart_post_survey_type.png}
%     \caption{User Rating Mean}
%     \label{fig:bar_response}
%     \end{subfigure}
%     \begin{subfigure}{0.40\textwidth}
%     % \centering
%     \includegraphics[height=2cm,keepaspectratio]{Figures/rating-chart/bar_chart_post_survey_stacked.png}
%     \caption{User Rating Stacked Bar}
%     \label{fig:bar_acc}
%     \end{subfigure}
%     \caption{The user rating towards different color palettes.\kenneth{TODOs: (1) The whole paper's figures should use the same color for Seq/Divergin/Qual bars. (2) The fonts of these figures should be larger. (3) Can you make these charts more flat by reducing the spaces between the bars?}\steven{done}}
%     \label{fig:user_rating}
% \end{figure*}

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016
modified by Matt Brehmer, Feb 2024

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE VIS: Visualization & Visual Analytics (Short Papers, Posters)
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Tables/table-color-acc-duration.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lcc}
    \toprule
& ACC   & Duration (sec) \\ \midrule
Sequential & .696 & 5.89         \\
Diverging & \textbf{.973} & 4.83         \\
Qualitative & .964 & 5.03         \\ \midrule
\textbf{Overall}         & .878 & 5.25 \\
\bottomrule
    \end{tabular}
    \caption{The accuracy and duration of each participant took with various color palettes. Participants had highest accuracy and spent the least amount of time on color palette 2.}
    \label{tab:color-palette-summary}
\end{table*}

==> Tables/table-post-survey.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{cccc}
    \toprule
{\multirow{2}{*}{\textbf{n=14}}} & {\multirow{2}{*}{\textbf{User Rate}}}   & \multicolumn{2}{c}{\textbf{T-test over Avg. User Rate}}\\ \cmidrule(lr){3-4}
\multicolumn{2}{c}{} & \multicolumn{1}{c}{Diverging} & \multicolumn{1}{c}{Qualitative}\\
\midrule
Sequential & 2.429	 &  <.001*** & <.001***        \\
Diverging & 4.643	 &  - &  .272       \\
Qualitative & 4.857 &  - &  -       \\ 
\bottomrule
    \end{tabular}
    \caption{Participants gave Sequential color palette significantly lower score than Diverging and Qualitative color palettes. }
     \vspace{-2pc}
    \label{tab:table-post-t-test}
\end{table*}


==> Tables/table-t-test-acc-between-colors.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{cccc}
    \toprule
{\multirow{2}{*}{\textbf{n=14}}} & {\multirow{2}{*}{\textbf{ACC}}}   & \multicolumn{2}{c}{\textbf{T-test over Avg. ACC}}\\ \cmidrule(lr){3-4}
\multicolumn{2}{c}{} & \multicolumn{1}{c}{Color-Palette-2} & \multicolumn{1}{c}{Color-Palette-3}\\
\midrule
Sequential & .696 &  <.001*** & <.001***        \\
Diverging & .973 &  - &  .720       \\
Qualitative & .964 &  - &  -       \\ 
\midrule
\textbf{Average} & .878 \\
\bottomrule
    \end{tabular}
    \caption{The Accuracy result of color palette study. Participants had highest accuracy on color palette 2. Color-Palette 1 is significantly worse than Color-Palette 2 and 3 on accuracy.}
    \label{tab:color-palette-acc-ttest}
\end{table*}

==> Tables/table-t-test-duration-time-between-colors.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{cccc}
    \toprule
{\multirow{2}{*}{\textbf{n=14}}} & {\multirow{2}{*}{\textbf{Duration (sec)}}}   & \multicolumn{2}{c}{\textbf{T-test over Avg. Duration}}\\ \cmidrule(lr){3-4}
\multicolumn{2}{c}{} & \multicolumn{1}{c}{Color-Palette-2} & \multicolumn{1}{c}{Color-Palette-3}\\
\midrule
Sequential & 5.89 &  <.001*** & <.001***        \\
Diverging & 4.83 &  - &  .271       \\
Qualitative & 5.03 &  - &  -       \\ 
\midrule
Average & 5.25 \\
\bottomrule
    \end{tabular}
    \caption{The Duration result of color palette study. Participants spent the least amount of time on Color-Palette 2. Participants spent significantly more time on Color-Palette 1 than other color palettes.}
    \label{tab:color-palette-duration-ttest}
\end{table*}

==> Tables/table-t-test-response-rate-between-colors.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{cccc}
    \toprule
{\multirow{2}{*}{\textbf{n=14}}} & {\multirow{2}{*}{\textbf{Response Rate}}}   & \multicolumn{2}{c}{\textbf{T-test over Avg. Response Rate}}\\ \cmidrule(lr){3-4}
\multicolumn{2}{c}{} & \multicolumn{1}{c}{Color-Palette-2} & \multicolumn{1}{c}{Color-Palette-3}\\
\midrule
Sequential & .929	 &  .139 & .013*        \\
Diverging & .982	 &  - &  .583       \\
Qualitative & .991 &  - &  -       \\ 
\midrule
Average & .967 \\
\bottomrule
    \end{tabular}
    \caption{The Response Rate result of color palette study. Participants' response rate on Color-Palette 3 is significantly higher than that on Color-Palette 1. }
    \label{tab:color-palette-response-ttest}
\end{table*}

==> Tables/zero-shot-prompt-table.tex <==
\begin{table*}
\centering
    \begin{tabular}{@{}p{\textwidth}@{}}
        \hline
        \textbf{Zero-shot Prompt} \\
        Classify the given text into one of the following labels.\\ \\

        [Background]: Text segments answer one or more of these questions: Why is this problem important?,
        What relevant works have been created before?, What is still missing in the previous works?, 
        What are the high-level research questions?, How might this help other research or researchers?\\
        
        [Purpose]: Text segments answer one or more of these questions: What specific things do the researchers want to do?, What specific knowledge do the researchers want to gain?, What specific hypothesis do the researchers want to test?\\
        
        [Method]: Text segments answer one or more of these questions: How did the researchers do the work or find what they sought?, What are the procedures and steps of the research?\\
        
        [Finding]: Text segments answer one or more of these questions: What did the researchers find out?, Did the proposed methods work?, Did the thing behave as the researchers expected?
        
        [Other]: Text fragments that do NOT fit into any of the four categories above. Text fragments that are NOT part of the article. Text fragments that are NOT in English. Text fragments that contains ONLY reference marks (e.g., "[1,2,3,4,5") or ONLY dates (e.g., "April 20, 2008"). Captions for figures and tables (e.g. "Figure 1: Experimental Result of ...", or "Table 1: The Typical Symptoms of ...") Formatting errors. I really don't know or I'm not sure.\\ \\
        
        FAQs\\
        
        1. This text fragment has terms that I don't understand. What should I do? Please use the context in the article to figure out the focus. You can look up terms you don't know if you feel like you need to understand them.\\
        2. This text fragment is too short to mean anything. What should I do? If the text fragment is too short to have significant meanings, you could consider the entire sentence and answer based on the entire sentence.\\
        3. This text fragment is NOT in English. What should I do? If the whole fragment (or the majority of words in the fragment) is in Non-English, please label it as "Other". If the majority of the words in this fragment are in English with a few non-English words, please judge the label normally.\\
        4. I'm not sure if this should be a "background" or a "finding." How do I tell? When a sentence occurs in the earlier part of an article, and it is presented as a known fact or looks authoritative, it is often a "background" information.\\
        5. Do "potential applications of the proposed work" count as "background" or "purpose"? It should be "background." The "purpose" refers to specific things the paper wants to achieve.\\
        6. If the article says it's a "literature review" (e.g., "We reviewed the literature" / "In this article, we review.." etc), would we classify those as finding/contribution or purpose? Most parts of a literature review paper should still be "background" or "purpose", and only the "insight" drew from a set of prior works can be viewed as a "finding/contribution".\\
        7. What should I do with the case study on a patient? Typically, it has a patient come in with a set of signs and symptoms in the ER, and then the patient gets assessed and diagnosed. The patient is admitted to the hospital ICU and tests are done and they may be diagnosed with something else. In such cases, please label the interventions done by the medical staff (e.g., CT scans, X-rays, and medications given) as "Method", and the patient's final result (e.g. the patient's pneumonia resolved and he was released from the hospital) as "Finding/Contribution".\\ \\
        
        Classify the following sentence into one of the label: Background, Purpose, Method, Finding, and Other. \\Provide answer in format of ```fragment-i []''' \\

        fragment-1 Text: ```\{\textbf{Sentence-1}\}'''\\
        Label: []\\

        fragment-2 Text: ```\{\textbf{Sentence-2}\}'''\\
        Label: []\\

        fragment-3 Text: ```\{\textbf{Sentence-3}\}'''\\
        Label: []\\
        ......\\
        \hline
    \end{tabular}
    \caption{Zero-shot prompt used when calling GPT-4~\cite{he2024chi}.}
    \label{table:zero-shot-table}
\end{table*}


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

